Proviola: A Tool for Proof Re-animation

To improve on existing models of interaction with a proof assistant (PA), in particular for storage and replay of proofs, we in- troduce three related concepts, those of: a proof movie, consisting of frames which record both user input and the corresponding PA response; a camera, which films a user's interactive session with a PA as a movie; and a proviola, which replays a movie frame-by-frame to a third party. In this paper we describe the movie data structure and we discuss a proto- type implementation of the camera and proviola based on the ProofWeb system. ProofWeb uncouples the interaction with a PA via a web- interface (the client) from the actual PA that resides on the server. Our camera films a movie by "listening" to the ProofWeb communication. The first reason for developing movies is to uncouple the reviewing of a formal proof from the PA used to develop it: the movie concept enables users to discuss small code fragments without the need to install the PA or to load a whole library into it. Other advantages include the possibility to develop a separate com- mentary track to discuss or explain the PA interaction. We assert that a combined camera+proviola provides a generic layer between a client (user) and a server (PA). Finally we claim that movies are the right type of data to be stored in an encyclopedia of formalized mathematics, based on our experience in filming the Coq standard library.

==> figures/architecture.ltx <==
\begin{figure}
\begin{center}
\includegraphics[scale=.4]{figures/commMoviola}
\end{center}
\caption{Architectural overview of the moviola system.\label{fig:overview}}
\end{figure}


==> figures/commPW.ltx <==
\begin{figure}
  \begin{center}
    \includegraphics[scale=.4]{figures/commPW}
  \end{center}
  \caption{Communication using ProofWeb \label{fig:commpw}}
\end{figure}



==> figures/comm_trad.ltx <==
\begin{figure}
  \begin{center}
    \includegraphics[scale=.4]{figures/comm_trad}
  \end{center}
  \caption{Traditional communication of a proof\label{fig:commtrad}}
\end{figure}


==> figures/movEvolved.ltx <==
\begin{figure}
  \begin{center}
    \includegraphics[scale=.4]{figures/movEvolved}
  \end{center}
  \caption{Overview of the ProofWeb architecture using the camera as a Proxy\label{fig:movEvolved}}
\end{figure}


